Scalable Practical Synchronization of Heterogeneous Linear Systems

We study practical state synchronization of heterogeneous linear multi-agent systems over directed graphs using static diffusive state feedback. Persistent mismatches between the agent dynamics generally preclude exact synchronization and are treated as bounded disturbances within an Input-to-State Stability (ISS) framework. We derive a scalable synthesis procedure based on fixed-dimension linear matrix inequalities (LMIs), whose dimension is independent of the number of agents. Local robust dissipation conditions are combined through a small-gain argument to obtain global ISS guarantees and explicit bounds on the synchronization error. The framework is formulated in a unified manner for continuous- and discrete-time systems, while highlighting a fundamental difference in disturbance attenuation between the two domains. In particular, exact ZOH discretization of a continuous-time controller need not preserve closed-loop stability, motivating a native discrete-time synthesis. Numerical experiments on heterogeneous harmonic oscillators illustrate the proposed approach and the continuous/discrete-time distinction.

==> sections/NumericalExample.tex <==
\section{Numerical Example}

\label{section:numerical_example}

In this section, we validate the theoretical results established in Section~\ref{sec:main_results} through a practical synchronization problem. We consider a heterogeneous network of linear harmonic oscillators to demonstrate the effectiveness of both the proposed Continuous-Time (CT) and Discrete-Time (DT) control designs. For each domain, we compare the open-loop (uncontrolled) and closed-loop state trajectories, together with the resulting average synchronization error, to quantify the benefit of the proposed diffusive coupling. Furthermore, we highlight the structural limitations of applying a discretized CT controller under larger sampling periods, thereby emphasizing the necessity and robustness of the native DT synthesis developed in Proposition~\ref{prop:DT_LMI}.

\subsection{Network Description}

Consider a multi-agent system composed of $N=6$ follower agents and one virtual leader (Agent 0). The agents are described by heterogeneous harmonic oscillators. 
%
The virtual leader oscillates at the nominal frequency $f_0 = 50\,\text{Hz}$ (i.e., $\omega_0 = 100\pi\,\text{rad/s}$). The followers exhibit parameter mismatches due to their natural frequencies $f_i$ being randomly drawn from a uniform distribution between $40\,\text{Hz}$ and $60\,\text{Hz}$. We define the nominal plant matrix $A$ based on the leader's dynamics, and the unstructured heterogeneity bound $\bar{\delta}$ is extracted dynamically via $\bar{\delta} = \max_{i} \|\Delta_i\|$. 

The communication topology between the leader and the 6 followers is modeled via a directed graph $\mathcal{G}$, as illustrated in Fig.~\ref{fig:network_topology}. This graph contains a directed spanning tree rooted at the virtual leader (Agent 0), ensuring that the leader's information can eventually reach all subsystems.

\begin{figure}[htpb]
    \centering
    \resizebox{0.8\columnwidth}{!}{%
    \begin{tikzpicture}[
        every node/.style={
            circle,
            draw,
            align=center,
            minimum size=1.2cm,
            font=\small
        },
        >=Stealth,
        scale=0.9
    ]

    % Leader (soft red)
    \node[fill={rgb,1:red,0.85;green,0.35;blue,0.35}, thick] (1) at (0,5) {\textbf{(0)} \\ 50 Hz};

    % Nodes (desaturated / pastel versions)
    \node[fill={rgb,1:red,0.85;green,0.65;blue,0.45}] (2) at (-4,3) {\textbf{(1)} \\ 53 Hz};
    \node[fill={rgb,1:red,0.90;green,0.82;blue,0.55}] (3) at (4,3) {\textbf{(2)} \\ 41 Hz};

    \node[fill={rgb,1:red,0.70;green,0.50;blue,0.85}] (7) at (-2,1) {\textbf{(6)} \\ 56 Hz};
    \node[fill={rgb,1:red,0.55;green,0.80;blue,0.55}] (4) at (2,1) {\textbf{(3)} \\ 60 Hz};
    \node[fill={rgb,1:red,0.60;green,0.88;blue,0.95}] (5) at (-2,-1) {\textbf{(4)} \\ 40 Hz};
    \node[fill={rgb,1:red,0.85;green,0.45;blue,0.70}] (6) at (2,-1) {\textbf{(5)} \\ 42 Hz};

    % Edges
    \draw[->] (1) -- (2);
    \draw[->] (1) -- (3);
    \draw[->] (1) to[bend left=15] (4);

    \draw[->] (2) to[bend left=10] (4);
    \draw[->] (2) to[bend right=10] (5);

    \draw[->] (3) to[bend left=5] (6);
    \draw[->] (3) .. controls (4.5,-2.2) and (1.5,-3.2) .. (5);

    % cycle highlight
    \draw[->, very thick, red, rounded corners=8pt] (5) -- (7);
    \draw[->, very thick, red, rounded corners=8pt] (7) -- (4);
    \draw[->, very thick, red, rounded corners=8pt] (4) -- (6);
    \draw[->, very thick, red, rounded corners=8pt] (6) -- (5);

    \end{tikzpicture}
    }
    \caption{Directed communication graph topology $\mathcal{G}$ representing the interaction between the virtual leader (Agent 0) and the $N=6$ heterogeneous followers.}
    \label{fig:network_topology}
\end{figure}

\subsection{Continuous-Time Design}

The continuous-time local dynamics for the heterogeneous harmonic oscillators are given by:
\begin{equation}
    \label{eq:oscillator_models}
    \dot{x}_i = \begin{bmatrix}
        0 & \omega_i\\ -\omega_i & 0
    \end{bmatrix}x_i + \begin{bmatrix}
        0\\ 1
    \end{bmatrix}u_i.
\end{equation}

The synthesis of the feedback gain $K_{\text{CT}}$ relies on the robust dissipation framework established in Proposition~\ref{prop:CT_LMI} to guarantee stability under the specified heterogeneity bounds ($\bar{\delta}=62.8319$). 
The feasible solution yields the stabilizing control gain:
\begin{equation}
    K_{\text{CT}} = \begin{bmatrix} -479.5712 & -906.0123 \end{bmatrix},
\end{equation}
with the associated Lyapunov matrix $P$ and synthesis scalars:
\begin{equation*}
    P = 10^7 \begin{bmatrix}
    7.6550  &  3.9259 \\
    3.9259  &  7.3685
    \end{bmatrix}, \quad \gamma = 2.0368,
\end{equation*}
\begin{equation*}
    \eta = 6.5076 \times 10^{4}, \quad \alpha = 11.0009, \quad \tau = 7.2585 \times 10^{-7}.
\end{equation*}

These synthesis parameters satisfy the small-gain condition \eqref{eq:small_gain_condition} of Theorem \ref{th:main_theorem} for the network topology in Fig. \ref{fig:network_topology}, thereby guaranteeing practical synchronization of the continuous-time network.

To assess the effectiveness of the proposed diffusive coupling, we compare the open-loop network, in which each follower evolves in isolation ($u_i \equiv 0$) and merely oscillates at its own mismatched frequency $\omega_i$, with the closed-loop network under the synthesized gain $K_{\text{CT}}$. Fig.~\ref{fig:ct_avg_error} depicts the resulting state trajectories $x_i(t)$ in both regimes: in open loop the agents drift apart due to the frequency mismatch, whereas in closed loop they remain locked to a common oscillatory pattern dictated by the leader. To quantify this behavior, Fig.~\ref{fig:ct_avg_error} also reports the average synchronization error $\bar e(t) := \frac{1}{N}\sum_{i=1}^N \|e_i(t)\|$ for both regimes: while the open-loop error persists at a level set by the uncompensated heterogeneity, the closed-loop error, consistently with Theorem~\ref{th:main_theorem}, converges to a bounded neighborhood of the origin, successfully achieving practical synchronization.

\begin{figure}[htpb]
    \centering
        \includegraphics[width=\columnwidth]{img/CT_plot.pdf}
    \caption{Comparison of open-loop and closed-loop state evolution $x_i(t)$ for the Continuous-Time (CT) design. Trajectory colors correspond to the node coloring defined in Fig.~\ref{fig:network_topology}, and the virtual leader (Agent 0) is highlighted in red. The average synchronization error $\bar e(t)$ is also shown for the open-loop and closed-loop CT designs.}
    \label{fig:ct_avg_error}
\end{figure}


\subsection{Discrete-Time Design}
\label{subsec:dt_design}

For a discrete implementation with a sampling frequency $f_s = 1\,\text{kHz}$ ($T_s = 1\,\text{ms}$), we utilize the native discrete-time framework established in Proposition~\ref{prop:DT_LMI}.

Before instantiating this synthesis, we address a structural issue that already arises at the modeling stage. The exact Zero-Order Hold (ZOH) discretization of the heterogeneous continuous-time oscillator \eqref{eq:oscillator_models} yields, for each agent $i$, a discrete-time model $x_i[k+1] = A_{d,i}x_i[k] + B_{d,i}u_i[k]$ with $A_{d,i} = e^{A_i T_s}$ and $B_{d,i} = \big(\int_0^{T_s} e^{A_i \tau}d\tau\big)B$. Since $A_i = A + \Delta_i$ depends on the agent's own frequency $\omega_i$, the exact input matrices are themselves heterogeneous, $B_{d,i} \neq B_{d,j}$ for $i \neq j$, which is incompatible with the common-input-matrix structure required by the unified synthesis of Section~\ref{sec:main_results}. To recover a common nominal input matrix, we evaluate it at the leader's nominal frequency $\omega_0$, obtaining a nominal matrix $B_d$, and absorb the residual mismatch into a scalar equalization factor $\phi_i$ such that $B_{d,i} \simeq \phi_i^{-1} B_d$. The discrete-time local model used for synthesis is thus

\begin{equation*}  \label{eq:dt_oscillator_models}
    \resizebox{\columnwidth}{!}{$
    x_i[k+1] = \begin{bmatrix}
        \cos(\omega_i T_s) & \sin(\omega_i T_s) \\
        -\sin(\omega_i T_s) & \cos(\omega_i T_s)
    \end{bmatrix} x_i[k] + \begin{bmatrix}
        \frac{1-\cos(\omega_0 T_s)}{\omega_0} \\
    \frac{\sin(\omega_0 T_s)}{\omega_0}
    \end{bmatrix} u_i[k],
    $}
\end{equation*}
and the implemented local control law is accordingly adapted to $u_i = \phi_i K_{\text{DT}} \sum_{j} a_{ij}(x_i - x_j)$, i.e., an individualized gain $K_i = \phi_i K_{\text{DT}}$, approximately compensating for the input mismatch while retaining the common Lyapunov certificate $P$ synthesized in Proposition~\ref{prop:DT_LMI}.

The synthesis of the feedback gain $K_{\text{DT}}$ relies on the robust dissipation framework established in Proposition~\ref{prop:DT_LMI} to guarantee stability under the specified discrete heterogeneity bound $\bar{\delta}=0.0628$.
The feasible solution yields the stabilizing control gain:
\begin{equation}
    K_{\text{DT}} = - \begin{bmatrix} 11.5933 & 221.8548 \end{bmatrix},
\end{equation}
with the associated Lyapunov matrix $P$ and synthesis scalars:
\begin{equation*}
    P = 10^4 \begin{bmatrix}
        4.9520 & 0.9400 \\
        0.9400 & 4.0458
    \end{bmatrix}, \quad \gamma = 0.0041,
\end{equation*}
\begin{equation*}
    \eta = 5.5644 \times 10^{4}, \quad \alpha = 0.1100, \quad \tau = 6.5356 \times 10^{-6}.
\end{equation*}

These synthesis parameters satisfy the small-gain condition \eqref{eq:small_gain_condition} of Theorem \ref{th:main_theorem} for the network topology in Fig. \ref{fig:network_topology}, thereby guaranteeing practical synchronization of the discrete-time network.

As in the continuous-time case, Fig.~\ref{fig:dt_avg_error} compares the open-loop ($u_i[k]\equiv 0$) and closed-loop state trajectories $x_i[k]$, Fig.~\ref{fig:dt_avg_error} also reports the corresponding average synchronization error $\bar e[k] := \frac{1}{N}\sum_{i=1}^N \|e_i[k]\|$. Consistently with Theorem~\ref{th:main_theorem}, the native DT design drives the average error to a bounded neighborhood of the origin, whereas in open loop the followers' states drift apart at their mismatched frequencies.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=\columnwidth]{img/DT_plot.pdf}
    \caption{Comparison of open-loop and closed-loop state evolution $x_i[k]$ for the native Discrete-Time (DT) design at $f_s = 1\,\text{kHz}$. Trajectory colors correspond to the node coloring defined in Fig.~\ref{fig:network_topology}, and the virtual leader (Agent 0) is highlighted in red. The average synchronization error $\bar e[k]$ is also shown for the open-loop and closed-loop DT designs.}
    \label{fig:dt_avg_error}
\end{figure}


\subsection{Discrete Implementation and CT Design Limitations}
\label{subsec:ct_limitations}

Discretely implementing the continuous-time synthesis via Zero-Order Hold (ZOH) introduces structural limitations, as plant discretization ($A_{d,i}$) alters the system's spectral properties. 

To illustrate this, we analyze the closed-loop spectrum of the aggregate error dynamics by varying the gain scaling factor $\kappa \in [0, 1]$ in the expression $(I_{N} \otimes A) + \Delta + (L_{22} \otimes \kappa BK)$. As depicted in Fig.~\ref{fig:eigenvalues_comparison}, we compare the eigenvalue distribution under three distinct scenarios:

\begin{itemize}
    \item Ideal CT Design (Fig.~\ref{fig:eigenvalues_comparison}a): The spectrum of the continuous closed-loop matrix using the exact continuous plant and the direct CT gain $K_{\text{CT}}$. The eigenvalues for $\kappa = 1$ lie strictly in the left half-plane, confirming the stability of the CT synthesis.
    
    \item discretized CT Design (Fig.~\ref{fig:eigenvalues_comparison}b): The spectrum of the true discretized plant $(A_{d,i}, B_{d,i})$ evaluated with the discretized CT controller $K_{\text{CT}}$. At $\kappa = 1$, several eigenvalues migrate outside the unit circle, indicating that the CT controller fails to stabilize the discrete plant.
    
    \item Native DT Design (Fig.~\ref{fig:eigenvalues_comparison}c): The spectrum utilizing the exact discretized plant $(A_{d,i}, B_{d,i})$, same sampling frequency as in the previous example, and the normalized native DT controller $K_i = \phi_i K_{\text{DT}}$ derived from Proposition~\ref{prop:DT_LMI}. The eigenvalues for $\kappa = 1$ remain safely constrained within the unit circle, validating the robustness of the discrete-time synthesis that natively accounts for the forward-shift operator dynamics.
\end{itemize}

\begin{figure}[htpb]
    \centering
    \begin{subfigure}[b]{0.98\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/eig_CT_CT.pdf}
        \caption{CT Plant ($A_i, B$) with CT Gain $K_{\text{CT}}$}
        \label{fig:eig_ct}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.98\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/eig_DT_CT.pdf}
        \caption{DT Plant ($A_{d,i}, B_{d,i}$) with CT Gain $K_{\text{CT}}$}
        \label{fig:eig_dt_kct}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.98\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/eig_DT_DT.pdf}
        \caption{DT Plant ($A_{d,i}, B_{d,i}$) with Scaled DT Gain $\phi_i K_{\text{DT}}$}
        \label{fig:eig_dt_kdt}
    \end{subfigure}
    \caption{Comparison of the closed-loop eigenvalue distribution for the synchronization error dynamics as $\kappa \in [0, 1]$ varies. The native DT design (c) inherently accounts for sample-and-hold dynamics and maintains stability inside the unit circle, whereas the discretized CT design (b) fails to preserve stability.}
    \label{fig:eigenvalues_comparison}
\end{figure}

==> sections/Solution.tex <==
\section{Main Results}

\label{sec:main_results}

In this section, we derive constructive conditions to synthesize the local feedback gain $K$ for the practical synchronization of heterogeneous multi-agent systems, as formulated in Problem \ref{prob:main_problem}. We employ the unified $\delta$-operator framework to provide a design approach valid for both continuous-time and discrete-time systems. We proceed in three steps. First, we provide general matrix inequality conditions guaranteeing dissipativity for a generic interconnection of linear subsystems (Lemma~\ref{lem:UnifiedDissipativityCondition}), and then adapt them to our setting through a scale-independent robust version tailored to the heterogeneous network structure (Lemma~\ref{lem:RobustUnifiedDissipativity}), which is subsequently linearized into tractable synthesis LMIs for the CT and DT domains (Propositions~\ref{prop:CT_LMI}--\ref{prop:DT_LMI}). Finally, we combine these local dissipativity certificates with the small-gain theorem to establish the main theorem, providing a solution to Problem~\ref{prob:main_problem} together with explicit ISS bounds on the synchronization error (Theorem~\ref{th:main_theorem}).

\subsection{Dissipativity Conditions}
\label{subsec:dissipativity}

We characterize the local stability properties of each follower agent by considering the general interconnected linear dynamics recalled in \eqref{eq:subsystem_dynamics}. By defining the aggregated vector of neighboring states $z_{-i} := \operatorname{col}(\{z_j\}_{j \neq i}) \in \mathbb{R}^{(N-1)n}$ and the stacked coupling matrix $\mathcal{G}_i := [G_{i1}, \dots, G_{i,i-1}, G_{i,i+1}, \dots, G_{iN}] \in \mathbb{R}^{n \times (N-1)n}$, the isolated subsystem dynamics can then be expressed in the standard interconnected form:
\begin{equation}
    \label{eq:subsystem_compact_generic}
    \delta z_i = F_i z_i + \mathcal{G}_i z_{-i} + C_i u_i.
\end{equation}
%
Furthermore, we define the block-diagonal interconnection gain matrix:
\[
    \Gamma_i := \operatorname{diag} \left( \gamma_{i1} P_1, \dots, \gamma_{i,i-1} P_{i-1}, \gamma_{i,i+1} P_{i+1}, \dots, \gamma_{iN} P_N \right),
\]
and introduce the structural matrix $\Phi$, defined to unify continuous-time (CT) and discrete-time (DT) domains:
\begin{equation}
    \label{eq:phi_definition}
    \Phi =
    \begin{cases}
        \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}, & \text{continuous-time (CT)}, \\[12pt]
        \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, & \text{discrete-time (DT)}.
    \end{cases}
\end{equation}

\begin{lemma}[Unified Dissipativity Condition]
\label{lem:UnifiedDissipativityCondition}
Consider subsystem $i$ described by \eqref{eq:subsystem_compact_generic}. For given scalars $\alpha_i > 0$, $\eta_i > 0$, $\gamma_{ij} \ge 0$, and the storage function $V_i(z_i) = z_i^\top P_i z_i$ with $P_i = P_i^\top \succ 0$, the dissipation inequality
\begin{equation}
    \label{eq:scalar_dissipation}
    \delta V_i \le -\alpha_i V_i(z_i) + \sum_{j \neq i} \gamma_{ij} V_j(z_j) + \eta_i |u_i|^2
\end{equation}
holds if and only if the following matrix inequality is satisfied:
\begin{equation}
    \label{eq:MI_dissipation}
    \begin{bmatrix} I & A_i^\top \\ 0 & \mathcal{B}_i^\top \\ 0 & E_i^\top \end{bmatrix} (\Phi \otimes P_i) \begin{bmatrix} I & 0 & 0 \\ A_i & \mathcal{B}_i & E_i \end{bmatrix} + \begin{bmatrix} \alpha_i P_i & 0 & 0 \\ 0 & -\Gamma_i & 0 \\ 0 & 0 & -\eta_i I \end{bmatrix} \preceq 0.
\end{equation}
\end{lemma}

\begin{proof}
For a quadratic function $V_i(z_i) = z_i^\top P_i z_i$, a direct computation of its variation yields the unified quadratic representation:
\begin{equation}
    \label{eq:deltaV_unified_quad}
    \delta V_i = \begin{pmatrix} z_i \\ \delta z_i \end{pmatrix}^{\!\top} (\Phi \otimes P_i) \begin{pmatrix} z_i \\ \delta z_i \end{pmatrix},
\end{equation}
where $\Phi$ is defined as in \eqref{eq:phi_definition}. 

Using the subsystem dynamics \eqref{eq:subsystem_compact_generic}, define the stacked vector $\xi_i := \operatorname{col}(z_i, z_{-i}, u_i)$ and the lifting matrix $\mathcal{M}_i := \begin{bmatrix} I & 0 & 0 \\ F_i & \mathcal{G}_i & C_i \end{bmatrix}$. Then $\operatorname{col}(z_i, \delta z_i) = \mathcal{M}_i \xi_i$, which implies $\delta V_i = \xi_i^\top \mathcal{M}_i^\top (\Phi \otimes P_i) \mathcal{M}_i \xi_i$. 

The inequality \eqref{eq:scalar_dissipation} can be rewritten as:
\[
    \delta V_i + \alpha_i V_i(z_i) - \sum_{j \neq i} \gamma_{ij} V_j(z_j) - \eta_i u_i^\top u_i \le 0.
\]
Substituting the quadratic forms $V_i(z_i) = \xi_i^\top \operatorname{diag}(P_i, 0, 0) \xi_i$, $\sum \gamma_{ij} V_j = \xi_i^\top \operatorname{diag}(0, \Gamma_i, 0) \xi_i$, and $u_i^\top u_i = \xi_i^\top \operatorname{diag}(0, 0, I) \xi_i$, we obtain:
\[
    \xi_i^\top \left( \mathcal{M}_i^\top (\Phi \otimes P_i) \mathcal{M}_i + \operatorname{diag}(\alpha_i P_i, -\Gamma_i, -\eta_i I) \right) \xi_i \le 0.
\]
Since this quadratic inequality must hold for all arbitrary vectors $\xi_i \in \mathbb{R}^{n + (N-1)n + m}$, it is satisfied if and only if the corresponding symmetric matrix is negative semi-definite, which is exactly the matrix inequality presented in \eqref{eq:MI_dissipation}.
\end{proof}

To decouple the dissipativity conditions from the network size $N$, we assume an interaction structure where the interconnection matrices decompose as $G_{ij} = a_{ij}B_i$, with $a_{ij} \ge 0$ being the scalar coupling weight from subsystem $j$ to subsystem $i$, and $B_i$ the input matrix of subsystem~$i$. We introduce the local aggregated interconnection variable:
\begin{equation}
    v_i := \sum_{j \neq i} a_{ij} x_j,
\end{equation}
which captures the total network influence on subsystem $i$ while preserving the state dimension. We restrict attention to the case where the dynamics of each subsystem are subject to a structured parameter variation $\beta_i T$, with scalar $\beta_i$ confined to the interval $[\beta_{\min}, \beta_{\max}]$ and known shape matrix $T \in \mathbb{R}^{n \times n}$, and to an unstructured heterogeneity $\Delta_i \in \mathbb{R}^{n \times n}$, described by the compact form
\begin{equation}
 \label{eq:robust_subsystem_dynamics}
    \delta x_i = (A + \beta_i T + \Delta_i) x_i + B_i v_i + E_i u_i,
\end{equation}
a structure chosen so as to later match, and thus be directly applicable to, the local error dynamics \eqref{eq:local_error_dynamics_final} of our synchronization problem. Here $\Delta_i$ represents an unstructured, norm-bounded heterogeneous uncertainty such that $\|\Delta_i\| \le \bar{\delta}$. To ensure the resulting matrix inequality is completely independent of the network size, we assume a homogeneous Lyapunov matrix $P = P^\top \succ 0$ across all subsystems: should $P_i$ be  allowed to vary with $i$, the interconnection block $\Gamma_i$ would in general require one copy of $P_j$ per neighbor $j$ of subsystem $i$, so that the size of the resulting matrix inequality would grow with the local degree of the network: precisely the scaling with $N$ we want to avoid.

\begin{lemma}[Robust scale-independent dissipativity condition]
\label{lem:RobustUnifiedDissipativity}
Consider subsystem $i$ described by \eqref{eq:robust_subsystem_dynamics} with parameter $\beta_i \in [\beta_{\min}, \beta_{\max}]$ and uncertainty $\|\Delta_i\| \le \bar{\delta}$. For given design scalars $\alpha > 0$, $\gamma > 0$, and $\eta > 0$, the dissipation inequality
\begin{equation}
    \label{eq:size_indep_scalar_dissipation_robust}
    \delta V_i(x_i) \le -\alpha V_i(x_i) + \gamma d_i \sum_{j \neq i} a_{ij} V_j + \eta \|u_i\|^2
\end{equation}
holds for all $\beta_i \in [\beta_{\min}, \beta_{\max}]$ and all $\|\Delta_i\| \le \bar{\delta}$ if there exists a scalar $\mu > 0$ such that the following fixed-dimension matrix inequality
\begin{equation}
    \label{eq:unified_robust_LMI}
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix} I & (A+\beta_i T)^\top \\ 0 & B_i^\top \\ 0 & E_i^\top \\ 0 & I \end{bmatrix} (\Phi \otimes P) \begin{bmatrix} I & 0 & 0 & 0 \\ A+\beta_i T & B_i & E_i & I \end{bmatrix} + \begin{bmatrix} \alpha P + \mu \bar{\delta}^2 I & 0 & 0 & 0 \\ 0 & -\gamma P & 0 & 0 \\ 0 & 0 & -\eta I & 0 \\ 0 & 0 & 0 & -\mu I \end{bmatrix} \preceq 0
    $}
\end{equation}
is satisfied at the vertices $\beta_i \in \{\beta_{\min}, \beta_{\max}\}$.
\end{lemma}

\begin{proof}
The proof is divided into three main parts: reformulating the uncertainty as an exogenous input, applying the S-procedure to embed the uncertainty bound, and verifying convexity with respect to the parameter $\beta_i$.

\textit{1. Uncertainty Reformulation.} Define the uncertain term as an additional exogenous input $w_i := \Delta_i x_i$. Since the uncertainty is norm-bounded ($\|\Delta_i\| \le \bar{\delta}$), this input satisfies the following quadratic constraint:
\[
    |w_i|^2 = x_i^\top \Delta_i^\top \Delta_i x_i \le \bar{\delta}^2 x_i^\top x_i \implies \bar{\delta}^2 x_i^\top x_i - w_i^\top w_i \ge 0.
\]
The subsystem dynamics can now be rewritten exactly as:
\[
    \delta x_i = (A + \beta_i T)x_i + B_i v_i + E_i u_i + I w_i.
\]
Define the augmented state vector $\tilde{\xi}_i := \operatorname{col}(x_i, v_i, u_i, w_i)$. We map $\tilde{\xi}_i$ to the state variation vector using the matrix $\mathcal{N}_i$:
\[
    \begin{bmatrix} x_i \\ \delta x_i \end{bmatrix} = 
    \begin{bmatrix} I & 0 & 0 & 0 \\ A+\beta_i T & B_i & E_i & I \end{bmatrix} \tilde{\xi}_i := \mathcal{N}_i \tilde{\xi}_i.
\]

\textit{2. Storage Function Variation and Interconnection Bounding.} Using the unified operator $\Phi$, the variation of the storage function is $\delta V(x_i) = \tilde{\xi}_i^\top \mathcal{N}_i^\top (\Phi \otimes P) \mathcal{N}_i \tilde{\xi}_i$. 

We now explicitly establish the upper bound for the aggregated interconnection term $v_i^\top P v_i$. Since $P \succ 0$ is symmetric, it admits a positive-definite square root $P^{1/2}$. Assuming the coupling weights are non-negative ($a_{ij} \ge 0$), we rewrite the quadratic form as the squared Euclidean norm of $P^{1/2} v_i$ and applying Cauchy-Schwarz inequality:
\begin{align*}
    v_i^\top P v_i &= \left\| P^{1/2} \sum_{j \neq i} a_{ij} x_j \right\|^2 = \left\| \sum_{j \neq i} \sqrt{a_{ij}} \left( \sqrt{a_{ij}} P^{1/2} x_j \right) \right\|^2 \\
    &\le \left( \sum_{j \neq i} \left(\sqrt{a_{ij}}\right)^2 \right) \left( \sum_{j \neq i} \left\| \sqrt{a_{ij}} P^{1/2} x_j \right\|^2 \right) \\
    &= \left( \sum_{j \neq i} a_{ij} \right) \left( \sum_{j \neq i} a_{ij} x_j^\top P x_j \right) = d_i \sum_{j \neq i} a_{ij} V_j.
\end{align*}
Substituting this estimate, the global dissipation inequality is guaranteed to be satisfied if the following stricter local condition holds:
\[
    \delta V(x_i) + \alpha x_i^\top P x_i - \gamma v_i^\top P v_i - \eta \|u_i\|^2 \le 0.
\]
Expressed in matrix form with respect to the augmented vector $\tilde{\xi}_i$, this requirement becomes:
\[
    \tilde{\xi}_i^\top \left[ \mathcal{N}_i^\top (\Phi \otimes P) \mathcal{N}_i + \operatorname{diag}(\alpha P, -\gamma P, -\eta I, 0) \right] \tilde{\xi}_i \le 0.
\]

\textit{3. S-Procedure and Vertex Condition.} The derived inequality must hold for all $\tilde{\xi}_i$ satisfying the uncertainty constraint $\tilde{\xi}_i^\top \operatorname{diag}(\bar{\delta}^2 I, 0, 0, -I) \tilde{\xi}_i \ge 0$. By the S-procedure (\cite{polik2007survey} Theorem 2.2), this is guaranteed if and only if there exists a scalar multiplier $\mu > 0$ such that:
\begin{multline*}
    \mathcal{N}_i^\top (\Phi \otimes P) \mathcal{N}_i + \operatorname{diag}(\alpha P, -\gamma P, -\eta I, 0) + \\ + \mu \operatorname{diag}(\bar{\delta}^2 I, 0, 0, -I) \preceq 0,
\end{multline*}
which directly yields the fixed-dimension matrix inequality~\eqref{eq:unified_robust_LMI}.

It remains to prove that verifying this MI at the vertices of $[\beta_{\min}, \beta_{\max}]$ is sufficient. Let $\mathcal{L}(\beta_i)$ denote the left-hand side of \eqref{eq:unified_robust_LMI}. The matrix $\mathcal{N}_i$ depends affinely on $\beta_i$ as $\mathcal{N}_i(\beta_i) = \mathcal{N}_0 + \beta_i \mathcal{N}_T$, where:
\[
    \mathcal{N}_0 = \begin{bmatrix} I & 0 & 0 & 0 \\ A & B_i & E_i & I \end{bmatrix}, \quad \text{and} \quad \mathcal{N}_T = \begin{bmatrix} 0 & 0 & 0 & 0 \\ T & 0 & 0 & 0 \end{bmatrix}.
\]
Substituting this into the leading quadratic term gives:
\begin{multline*}
    \mathcal{N}_i(\beta_i)^\top (\Phi \otimes P) \mathcal{N}_i(\beta_i) = \mathcal{N}_0^\top (\Phi \otimes P) \mathcal{N}_0 + \\ + \beta_i \operatorname{sym}\left( \mathcal{N}_0^\top (\Phi \otimes P) \mathcal{N}_T \right) + \beta_i^2 \mathcal{N}_T^\top (\Phi \otimes P) \mathcal{N}_T.
\end{multline*}

Because all other terms in $\mathcal{L}(\beta_i)$ are independent of $\beta_i$, the convexity of $\mathcal{L}(\beta_i)$ depends entirely on the quadratic coefficient block $\mathcal{Q} := \mathcal{N}_T^\top (\Phi \otimes P) \mathcal{N}_T$. Let us compute $\mathcal{Q}$ explicitly for both time domains:
\begin{itemize}
    \item In the continuous-time case, $\Phi \otimes P = \begin{bmatrix} 0 & P \\ P & 0 \end{bmatrix}$. Thus:
    \begin{multline*}
        \mathcal{Q} =
        \begin{bmatrix} 0 & T^\top \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \end{bmatrix}
        \begin{bmatrix} 0 & P \\ P & 0 \end{bmatrix}
        \begin{bmatrix} 0 & 0 & 0 & 0 \\ T & 0 & 0 & 0 \end{bmatrix}
        = \\ =
        \begin{bmatrix} T^\top P & 0 \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \end{bmatrix}
        \begin{bmatrix} 0 & 0 & 0 & 0 \\ T & 0 & 0 & 0 \end{bmatrix}
        = 0.
    \end{multline*}
    
    Since the quadratic term vanishes completely, $\mathcal{L}(\beta_i)$ is strictly \emph{affine} in $\beta_i$.
    
    \item In the discrete-time case, $\Phi \otimes P = \begin{bmatrix} -P & 0 \\ 0 & P \end{bmatrix}$. Thus:
    \begin{multline*}
            \mathcal{Q} =
            \begin{bmatrix} 0 & T^\top \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \end{bmatrix}
            \begin{bmatrix} -P & 0 \\ 0 & P \end{bmatrix}
            \begin{bmatrix} 0 & 0 & 0 & 0 \\ T & 0 & 0 & 0 \end{bmatrix}
            = \\ =
            \begin{bmatrix} 0 & T^\top P \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \end{bmatrix}
            \begin{bmatrix} 0 & 0 & 0 & 0 \\ T & 0 & 0 & 0 \end{bmatrix}
            =
            \begin{bmatrix} T^\top P T & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 \end{bmatrix}.
    \end{multline*}

    Since $P \succ 0$, it follows that $T^\top P T \succeq 0$, which means $\mathcal{Q} \succeq 0$. Therefore, for any fixed vector $\tilde{\xi}$, the mapping $\beta_i \mapsto \tilde{\xi}^\top \mathcal{L}(\beta_i) \tilde{\xi}$ is convex.
\end{itemize}

%\todo{MATH CHECK -- ho ricontrollato $\mathcal{Q}=\mathcal{N}_T^\top(\Phi\otimes P)\mathcal{N}_T$ a blocchi direttamente (senza passare dal prodotto intermedio) e i risultati finali sono corretti in entrambi i casi ($\mathcal{Q}=0$ in CT, $\mathcal{Q}=\operatorname{diag}(T^\top PT,0,0,0)$ in DT). Per\`o il passaggio intermedio mostrato mi pare abbia le entrate scambiate: $\begin{bmatrix}0 & T^\top\end{bmatrix}\begin{bmatrix}0&P\\P&0\end{bmatrix} = \begin{bmatrix}T^\top P & 0\end{bmatrix}$ (non $\begin{bmatrix}0 & T^\top P\end{bmatrix}$ come scritto) -- sembra un errore di trasposizione/ordine nel prodotto a blocchi mostrato in entrambi gli item (CT e DT). Non cambia le conclusioni finali, ma vale la pena sistemare il passaggio per chiarezza e correttezza, specie perch\'e con l'ordine scritto in bozza il prodotto finale con $\mathcal{N}_T$ darebbe $T^\top PT$ anche nel caso CT (cio\`e non tornerebbe pi\`u $\mathcal{Q}=0$), quindi il passaggio intermedio, cos\`i com'\`e, non supporta davvero la propria conclusione.}

A convex function defined over a compact interval $[\beta_{\min}, \beta_{\max}]$ must attain its maximum value at the boundary points. Consequently, enforcing $\mathcal{L}(\beta_{\min}) \preceq 0$ and $\mathcal{L}(\beta_{\max}) \preceq 0$ is necessary and sufficient to guarantee that $\mathcal{L}(\beta_i) \preceq 0$ holds for all intermediate values $\beta_i \in [\beta_{\min}, \beta_{\max}]$.
\end{proof}



\subsection{LMI Characterizations for Control Synthesis}

Starting from the local error dynamics \eqref{eq:local_error_dynamics_final}, and relabeling the leader-induced term $H_i x_0$ as a generic bounded disturbance $w_i$, the error dynamics of subsystem $i$ take the compact form
\begin{equation} \label{eq:error_dynamics}
    \delta e_i = (A + \Delta_i + d_i BK)e_i - BK \sum_{j \neq i}^N a_{ij} e_j + w_i.
\end{equation}
This expression instantiates the robust subsystem structure \eqref{eq:robust_subsystem_dynamics} of Lemma~\ref{lem:RobustUnifiedDissipativity} under the identification $\beta_i \equiv d_i$, $T \equiv BK$, $B_i \equiv -BK$, $E_i \equiv I$, $v_i \equiv \sum_{j\neq i} a_{ij}e_j$, and $u_i \equiv w_i$. The objective of this subsection is to provide tractable LMIs for the synthesis of the control gain $K$, obtained by specializing the robust scale-independent matrix inequality \eqref{eq:unified_robust_LMI} to this identification, for both the continuous-time and discrete-time domains.

\begin{proposition}[Continuous-Time LMI for dissipativity]
\label{prop:CT_LMI}
Consider the continuous-time error dynamics \eqref{eq:error_dynamics}. The system satisfies the robust scale-independent dissipation inequality \eqref{eq:size_indep_scalar_dissipation_robust} if there exist $X = X^\top \succ 0$, $Y$, and $\tau > 0$ such that, for all vertices $d_i \in \{d_{\min}, d_{\max}\}$, the following LMI holds:
\begin{equation}
    \label{eq:CT_LMI_final}
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        \mathrm{sym}(AX + d_i BY) + \alpha X & -BY & I & \tau I & \bar{\delta} X \\
        -Y^\top B^\top & -\gamma X & 0 & 0 & 0 \\
        I & 0 & -\eta I & 0 & 0 \\
        \tau I & 0 & 0 & -\tau I & 0 \\
        \bar{\delta} X & 0 & 0 & 0 & -\tau I
    \end{bmatrix} \preceq 0,
    $}
\end{equation}
where the stabilizing feedback control gain is recovered via $K = Y X^{-1}$.
\end{proposition}

\begin{proof}

The proof proceeds by linearizing the robust dissipativity condition through a sequence of matrix transformations.

Under the identification established in \eqref{eq:error_dynamics} ($\beta_i \equiv d_i$, $T \equiv BK$, $B_i \equiv -BK$, $E_i \equiv I$), the continuous-time robust condition \eqref{eq:unified_robust_LMI} instantiates to a Bilinear Matrix Inequality (BMI), which is non-linear due to the coupling between $P$ and $K$:
$$
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        \mathrm{sym}(P(A+d_i BK)) + \alpha P + \mu \bar{\delta}^2 I & -PBK & P & P \\
        -K^\top B^\top P & -\gamma P & 0 & 0 \\
        P & 0 & -\eta I & 0 \\
        P & 0 & 0 & -\mu I
    \end{bmatrix} \preceq 0.
    $}
$$

To decouple the variables, we introduce the congruence transformation matrix $\Pi_{\mathrm{CT}} = \operatorname{diag}(P^{-1}, P^{-1}, I, I)$. Pre- and post-multiplying the BMI by $\Pi_{\mathrm{CT}}$ and applying the standard changes of variables $X := P^{-1}$ and $Y := KX$ results in:
$$
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        \mathrm{sym}(AX + d_i BY) + \alpha X + \mu \bar{\delta}^2 X^2 & -BY & I & I \\
        -Y^\top B^\top & -\gamma X & 0 & 0 \\
        I & 0 & -\eta I & 0 \\
        I & 0 & 0 & -\mu I
    \end{bmatrix} \preceq 0.
    $}
$$

The matrix is still non-linear due to the quadratic term $\mu \bar{\delta}^2 X^2$ in the $(1,1)$ block. We rewrite this term as $(\bar{\delta} X) (\mu^{-1} I)^{-1} (\bar{\delta} X)$ and apply the Schur complement to isolate the uncertainty. This expands the inequality into a $5 \times 5$ block matrix:
$$
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        \mathrm{sym}(AX + d_i BY) + \alpha X & -BY & I & I & \bar{\delta}X \\
        -Y^\top B^\top & -\gamma X & 0 & 0 & 0 \\
        I & 0 & -\eta I & 0 & 0 \\
        I & 0 & 0 & -\mu I & 0 \\
        \bar{\delta}X & 0 & 0 & 0 & -\mu^{-1} I
    \end{bmatrix} \preceq 0.
    $}
$$

To eliminate the inverse dependencies between $\mu$ and $\mu^{-1}$, we introduce the scalar parameter $\tau := \mu^{-1}$. Finally, we apply a partial congruence transformation by multiplying the fourth row and column by $\tau$. This scales the $(1,4)$ and $(4,1)$ blocks to $\tau I$, transforms the $(4,4)$ block from $-\mu I$ to $-\mu \tau^2 I = -\tau I$, and maps the $(5,5)$ block directly to $-\tau I$. This completely linearizes the system, yielding LMI \eqref{eq:CT_LMI_final}.
\end{proof}

\begin{proposition}[Discrete-Time LMI for dissipativity]
\label{prop:DT_LMI}
Consider the discrete-time error dynamics \eqref{eq:error_dynamics}. The system satisfies the robust scale-independent dissipation inequality \eqref{eq:size_indep_scalar_dissipation_robust} if there exist $X = X^\top \succ 0$, $Y$, and $\tau > 0$ such that, for all vertices $d_i \in \{d_{\min}, d_{\max}\}$, the following LMI holds:
\begin{equation}
    \label{eq:DT_LMI_final}
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        (\alpha - 1)X & 0 & 0 & X A^\top + d_i Y^\top B^\top & 0 & \bar{\delta} X \\
        0 & -\gamma X & 0 & -Y^\top B^\top & 0 & 0 \\
        0 & 0 & -\eta I & I & 0 & 0 \\
        A X + d_i B Y & -B Y & I & -X & \tau I & 0 \\
        0 & 0 & 0 & \tau I & -\tau I & 0 \\
        \bar{\delta} X & 0 & 0 & 0 & 0 & -\tau I
    \end{bmatrix} \preceq 0,
    $}
\end{equation}
where the stabilizing feedback control gain is recovered via $K = Y X^{-1}$.
\end{proposition}

\begin{proof}

Paralleling the continuous-time case, we derive the LMI through a four-step linearization process.

Under the identification established in \eqref{eq:error_dynamics} ($\beta_i \equiv d_i$, $T \equiv BK$, $B_i \equiv -BK$, $E_i \equiv I$), the discrete-time robust condition \eqref{eq:unified_robust_LMI}, after applying the Schur complement, instantiates to the BMI:
$$
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        (\alpha - 1) P + \mu \bar{\delta}^2 I & 0 & 0 & (A+d_i BK)^\top P & 0 \\
        0 & -\gamma P & 0 & -K^\top B^\top P & 0 \\
        0 & 0 & -\eta I & P & 0 \\
        P(A+d_i BK) & -PBK & P & -P & P \\
        0 & 0 & 0 & P & -\mu I
    \end{bmatrix} \preceq 0.
    $}
$$

We apply the congruence matrix $\Pi_{\mathrm{DT1}} = \operatorname{diag}(P^{-1}, P^{-1}, I, P^{-1}, I)$. Setting $X := P^{-1}$ and $Y := KX$, this transformation partially decouples the variables, yielding:
$$
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        (\alpha - 1)X + \mu \bar{\delta}^2 X^2 & 0 & 0 & X A^\top + d_i Y^\top B^\top & 0 \\
        0 & -\gamma X & 0 & -Y^\top B^\top & 0 \\
        0 & 0 & -\eta I & I & 0 \\
        A X + d_i B Y & -B Y & I & -X & I \\
        0 & 0 & 0 & I & -\mu I
    \end{bmatrix} \preceq 0.
    $}
$$

This inequality exhibits two coupled non-linearities: the quadratic term $\mu \bar{\delta}^2 X^2$ in the $(1,1)$ block, and the linear term $-\mu I$ in the $(5,5)$ block. We define the parameter inversion $\tau := \mu^{-1}$, which transforms the $(1,1)$ non-linearity into $\tau^{-1} (\bar{\delta}X) I (\bar{\delta}X)$ and the $(5,5)$ block into $-\tau^{-1} I$.

Applying the Schur complement to the $(1,1)$ term expands the matrix to a $6 \times 6$ structure. The new $(6,6)$ block becomes $-\tau I$, and the coupling block at $(1,6)$ becomes $\bar{\delta}X$:
$$
    \resizebox{\columnwidth}{!}{$
    \begin{bmatrix}
        (\alpha - 1)X & 0 & 0 & X A^\top + d_i Y^\top B^\top & 0 & \bar{\delta} X \\
        0 & -\gamma X & 0 & -Y^\top B^\top & 0 & 0 \\
        0 & 0 & -\eta I & I & 0 & 0 \\
        A X + d_i B Y & -B Y & I & -X & I & 0 \\
        0 & 0 & 0 & I & -\tau^{-1} I & 0 \\
        \bar{\delta} X & 0 & 0 & 0 & 0 & -\tau I
    \end{bmatrix} \preceq 0.
    $}
$$

To resolve the remaining $\tau^{-1}$ inversion in the fifth diagonal block, we apply a final partial congruence transformation via $\Pi_{\mathrm{DT2}} = \operatorname{diag}(I, I, I, I, \tau I, I)$. Scaling the fifth row and column by $\tau$ shifts the $(4,5)$ and $(5,4)$ positions from $I$ to $\tau I$, and scales the $(5,5)$ block from $-\tau^{-1} I$ to $-\tau I$. This completely linearizes the matrix inequality, directly recovering the valid synthesis LMI \eqref{eq:DT_LMI_final}.

\end{proof}


\subsection{Synchronization Result}

Consider the network of $N$ heterogeneous subsystems governed by the error dynamics \eqref{eq:error_dynamics}, where $e_i$ is the local tracking error, $w_i$ is a bounded external disturbance (as a consequence of Assumption \ref{ass:bounded_heterogeneity} and \ref{ass:leader_trajectory}), $d_i$ is the local topological coupling degree, and $\Delta_i$ represents parametric heterogeneity such that $\|\Delta_i\| \le \bar{\delta}$. Let $e = \operatorname{col}(e_1, \dots, e_N)$ and $w = \operatorname{col}(w_1, \dots, w_N)$ denote the global error and disturbance vectors.

The following theorem establishes conditions for practical synchronization under this unified dynamics and provides explicit ISS bounds. 



\begin{theorem}[Practical Synchronization]
\label{th:main_theorem}
Consider the interconnected network \eqref{eq:error_dynamics}. Suppose there exist a common Lyapunov matrix $P \succ 0$, a control gain $K$, and positive scalars $\alpha$, $\gamma$, and $\eta$ such that the LMI \eqref{eq:CT_LMI_final} for continuous-time, or \eqref{eq:DT_LMI_final} for discrete-time, is feasible. If the network interconnection satisfies the small-gain condition:
\begin{equation}
    \label{eq:small_gain_condition}
    \gamma < \frac{\alpha}{\rho(D\mathcal{A})},
\end{equation}
where $D = \operatorname{diag}(d_1, \dots, d_N)$ and $\mathcal{A} = [a_{ij}]$, then the network achieves practical synchronization. The global error $e$ is Input-to-State Stable (ISS) with respect to $w$, satisfying:
\begin{equation}
    \|e(\mathfrak{t})\|^2 \le \kappa \beta(\mathfrak{t}) \|e(0)\|^2 + \zeta \sup_{s \in \mathcal{I}_\mathfrak{t}} \|w(s)\|_{\infty}^2,
\end{equation}
    
where $\mathfrak{t}$, $\beta(\mathfrak{t})$, and $\mathcal{I}_\mathfrak{t}$ are defined as:
\begin{itemize}
    \item Continuous-Time: $\mathfrak{t} = t \in\mathbb{R}_{\ge 0}$, $\beta(t) = e^{-\theta \alpha t}$, $\mathcal{I}_t = [0, t]$.
    \item Discrete-Time: $\mathfrak{t} = k \in\mathbb{Z}_{\ge 0}$, $\beta(k) = (1 - \theta \alpha)^k$, $\mathcal{I}_k = \{0, 1, \dots, k-1\}$.
\end{itemize}
Here $c \in \mathbb{R}^N$ is any vector such that $\frac{\gamma}{\alpha} D\mathcal{A}\, c < c$; and
\begin{align*}
    \theta &= \min_i \left(1 - \frac{\gamma}{\alpha}\frac{d_i \sum_{j\neq i} a_{ij}c_j}{c_i}\right) \in (0,1], \\
    \kappa &= \frac{N c_{\max} \lambda_{\max}(P)}{c_{\min} \lambda_{\min}(P)}, \\
    \zeta &= \frac{N c_{\max} \eta}{\theta \alpha c_{\min} \lambda_{\min}(P)},
\end{align*}
    
with $c_{\max} = \max_i c_i$, $c_{\min} = \min_i c_i$.
\end{theorem}


\begin{proof}
Let $V_i(e_i) = e_i^\top P e_i$ be the local ISS-Lyapunov candidate function. The feasibility of \eqref{eq:CT_LMI_final}--\eqref{eq:DT_LMI_final} guarantees the local dissipation inequality:
\[
    \delta V_i \le -\alpha V_i + \gamma d_i \sum_{j \neq i}^N a_{ij} V_j + \eta \|w_i\|^2.
\]
The condition $\gamma < \frac{\alpha}{\rho(D\mathcal{A})}$ implies 
$\rho\!\left(\frac{\gamma}{\alpha}D\mathcal{A}\right)<1$. Since 
$\frac{\gamma}{\alpha}D\mathcal{A}\ge0$ entrywise, this guarantees 
(see Remark \ref{rem:construction_c}) the existence of a strictly positive 
vector $c=[c_1,\dots,c_N]^\top>0$ such that
\[
    \frac{\gamma}{\alpha}D\mathcal{A}c<c .
\]
Equivalently, the above inequality holds componentwise as
\[
    \frac{\gamma}{\alpha}d_i\sum_{j\neq i}a_{ij}c_j<c_i,
    \qquad i=1,\dots,N .
\]
Therefore, we may define
\[
    \theta:=\min_i\left(1-\frac{\gamma}{\alpha}
    \frac{d_i\sum_{j\neq i}a_{ij}c_j}{c_i}\right)\in(0,1],
\]
which yields the bound
\begin{equation}
    \gamma d_i \sum_{j\neq i}^N a_{ij} c_j
    \;\le\; \alpha(1-\theta)c_i,
    \qquad i=1,\dots,N .
    \label{eq:interconnection_bound}
\end{equation}

We construct the global ISS-Lyapunov function $V(e) = \max_{i} \{V_i(e_i)/c_i\}$. Given the bounds $\lambda_{\min}(P)\|e_i\|^2 \le V_i \le \lambda_{\max}(P)\|e_i\|^2$, the global function satisfies:
\[
    \frac{\lambda_{\min}(P)}{N c_{\max}} \|e\|^2 \le V(e) \le \frac{\lambda_{\max}(P)}{c_{\min}} \|e\|^2.
\]
Let $m$ be the index of the active subsystem such that $V(e) = V_m(e_m)/c_m$. The unified variation $\delta V(e)$ satisfies:
\begin{align*}
    \delta V(e) &= \frac{\delta V_m}{c_m} \le -\alpha \frac{V_m}{c_m} + \frac{\gamma d_m}{c_m} \sum_{j \neq m}^N a_{mj} V_j + \frac{\eta}{c_m} \|w_m\|^2 \\
    &\le -\alpha V(e) + \gamma d_m \sum_{j \neq m}^N a_{mj} \frac{c_j}{c_m} V(e) + \frac{\eta}{c_{\min}} \|w\|_{\infty}^2 \\
    &\le -\alpha V(e) + \alpha(1-\theta) V(e) + \frac{\eta}{c_{\min}} \|w\|_{\infty}^2 \\
    &= -\theta \alpha V(e) + \frac{\eta}{c_{\min}} \|w\|_{\infty}^2,
\end{align*}
where the second to last step uses $V_j \le c_j V(e)$ for all $j$ (by definition of $V$ as the max) together with \eqref{eq:interconnection_bound} divided by $c_m$.

In the continuous-time case, $V$ is locally Lipschitz but non-differentiable where the active index $m$ switches; since the bound above holds for every active $V_i$, it holds for every element of the Clarke generalized gradient of $V$, exactly as argued in the proof of \cite[Thm. 11]{dashkovskiy2007iss}, to which we refer for details.


\textit{Continuous-Time Case ($\delta = d/dt$):} The inequality $\dot{V} \le -\theta \alpha V + \frac{\eta}{c_{\min}} \|w\|_{\infty}^2$ is a linear differential inequality. By the Comparison Lemma:
\begin{multline*}
    V(e(t)) \le e^{-\theta \alpha t} V(e(0)) + \frac{\eta}{c_{\min}} \int_0^t e^{-\theta \alpha (t-s)} \|w(s)\|^2 ds \le\\ e^{-\theta \alpha t} V(e(0)) + \frac{\eta}{\theta \alpha c_{\min}} \sup_{0 \le s \le t} \|w(s)\|^2.
\end{multline*}

\textit{Discrete-Time Case ($\delta V = V(k+1)-V(k)$):} The inequality $V(k+1) \le (1-\theta \alpha)V(k) + \frac{\eta}{c_{\min}} \|w\|_{\infty}^2$ implies:
\[
    V(k) \le (1-\theta \alpha)^k V(0) + \frac{\eta}{c_{\min}} \sum_{s=0}^{k-1} (1-\theta \alpha)^{k-1-s} \|w(s)\|^2.
\]
Bounding the geometric series $\sum_{j=0}^{k-1} (1-\theta \alpha)^j \le \frac{1}{\theta \alpha}$, we obtain:
\[
    V(k) \le (1-\theta \alpha)^k V(0) + \frac{\eta}{\theta \alpha c_{\min}} \sup_{0 \le s \le k-1} \|w(s)\|^2.
\]
Substituting the global norm bounds for $V(e)$ into the respective time-domain solutions yields the final ISS estimates for both domains.
\end{proof}

\begin{remark}[Optimal Selection of $c$]
\label{rem:optimal_c}
Theorem \ref{th:main_theorem} holds for any $c>0$ satisfying $\frac{\gamma}{\alpha}D\mathcal{A}c<c$, but $\theta$ depends on this choice and governs the convergence rate. Writing $\Gamma:=\frac{\gamma}{\alpha}D\mathcal{A}\ge 0$, we have $\theta(c) = 1-\max_i (\Gamma c)_i/c_i$, so maximizing $\theta$ is equivalent to the minimization $\rho(\Gamma) = \min_{c>0}\max_i (\Gamma c)_i/c_i$.

\textit{Irreducible case.} If $\mathcal{A}$ induces a strongly connected graph, $\Gamma$ is irreducible and admits a strictly positive Perron eigenvector $v>0$ with $\Gamma v=\rho(\Gamma)v$. Choosing $c=v$ yields the optimal rate $\theta^\star=1-\rho(\Gamma)=1-\frac{\gamma}{\alpha}\rho(D\mathcal{A})$, matching the residual margin in the small-gain condition.

\textit{Reducible case.} If $\mathcal{A}$ is reducible, the Perron eigenvector of $\Gamma$ may have zero entries and is thus inadmissible. We instead perturb: for $\varepsilon>0$, let $\Gamma_\varepsilon:=\Gamma+\varepsilon\mathbf{1}\mathbf{1}^\top$, which is irreducible and admits $v_\varepsilon>0$ with $\Gamma_\varepsilon v_\varepsilon=\rho(\Gamma_\varepsilon)v_\varepsilon$, where $\rho(\Gamma_\varepsilon)\to\rho(\Gamma)$ as $\varepsilon\to0^+$. Since $\Gamma\le \Gamma_\varepsilon$ entrywise, $\Gamma v_\varepsilon\le\rho(\Gamma_\varepsilon)v_\varepsilon$, so $c=v_\varepsilon$ is admissible and gives $\theta(v_\varepsilon)\ge 1-\rho(\Gamma_\varepsilon)$, arbitrarily close to $\theta^\star$ for small $\varepsilon$.
\end{remark}


The proposed synthesis requires only high-level knowledge of the network topology through the quantities entering the small gain condition ($\rho(D\mathcal{A})$) and the LMIs ($d_i$). If exact network information is unavailable, conservative estimates of the graph parameters can be employed, at the price of increased conservatism in the achievable performance bounds. On the other hand, this conservatism provides additional robustness against uncertainties in the network topology, ensuring that the synchronization guarantees remain valid even when the actual interconnection differs from the nominal one. It is worth emphasizing that the Perron-Frobenius vector is only required for the stability analysis and does not enter the controller implementation.


The ISS gain $\zeta$ explicitly quantifies the steady-state synchronization accuracy achieved by the network. In particular, since $\theta\ge 1-\frac{\gamma}{\alpha}\rho(D\mathcal A)$, the gain $\zeta$ depends both on design parameters ($P$, $\alpha$, $\gamma$, $\eta$) and on the network topology ($\mathcal{A}$). A larger decay rate~$\alpha$, a smaller disturbance gain~$\eta$, and a larger stability margin~$\theta$ all reduce $\zeta$, leading to tighter synchronization. 
The gain $\zeta$ can be made arbitrarily small only for CT dynamics, as we discuss in the following remark.


\begin{remark}[Continuous vs. Discrete-Time Asymmetry and Structural Limitations]
For a generic LTI system $\delta e = A_{\text{cl}} e + w$, subject to a persistent disturbance $w$, steady-state attenuation is governed by the static sensitivity matrix: $-A_{\text{cl}}^{-1}$ in continuous-time (CT) and $(I - A_{\text{cl}})^{-1}$ in discrete-time (DT). In CT, shifting eigenvalues arbitrarily far into the left half-plane ($\Re(\lambda) \to -\infty$) drives $\|A_{\text{cl}}^{-1}\| \to 0$, enabling arbitrary disturbance attenuation. Conversely, in DT, asymptotic stability strictly confines eigenvalues inside the unit circle ($|\lambda| < 1$), bounding the spectral distance $|1 - \lambda| < 2$. Thus, $\|(I - A_{\text{cl}})^{-1}\|$ cannot be made arbitrarily small, imposing an unavoidable structural floor on DT accuracy.

This principle applies directly to our collective error dynamics (25), governed by the open-loop pair $(I_N \otimes A) + \Delta = \operatorname{blkdiag}(A_1, \dots, A_N)$ and $L_{22} \otimes B$. While arbitrary error reduction via an unrestricted controller only requires standard controllability of this pair, our protocol enforces a replicated, block-diagonal structure $I_N \otimes K$.
Because a single static gain $K$ must simultaneously stabilize and tune the decay rate $\alpha$ across all heterogeneous agents, driving the CT error bound $\zeta$ in Theorem~1 to zero is far more restrictive than standard controllability, which is the price to pay for obtaining a synthesis independent of the network size. It requires either full actuation ($\operatorname{rank}(B) = n$) or matched heterogeneity $A_i = A_0 + B \tilde\Delta_i$ for some matrices $\tilde\Delta_i \in \mathbb{R}^{m \times n}$. Even when these stringent structural conditions are met, the DT synchronization error remains inherently bounded due to the unit-circle confinement.
\end{remark}

Theorem~\ref{th:main_theorem} provides an ISS bound with respect to the aggregate disturbance $w$. Since, in the synchronization problem, this disturbance is induced by the mismatch between the follower and leader dynamics, the result can be specialized directly to the leader state as follows.

\begin{corollary}
    Under the condition of Theorem~\ref{th:main_theorem}, the aggregate error system \eqref{eq:global_error_system} is ISS with respect to the leader state $x_0$, in the sense of Definition~\ref{def:practical_sync}. In particular,
    \begin{equation}
        \label{eq:iss_x0_bound}
        \|e(\mathfrak{t})\|^2 \le \kappa \beta(\mathfrak{t})\|e(0)\|^2 + 4\bar\delta^2\zeta \sup_{s\in\mathcal{I}_\mathfrak{t}}\|x_0(s)\|^2
    \end{equation}
    with $\mathfrak{t}$, $\beta(\mathfrak{t})$, $\mathcal{I}_\mathfrak{t}$ as in Theorem~\ref{th:main_theorem}.
\end{corollary}
\begin{proof}
    By construction $w_i=H_i x_0$ with $H_i=\Delta_i-\Delta_0$. Under Assumption~\ref{ass:bounded_heterogeneity}, $\|H_i\|\le\|\Delta_i\|+\|\Delta_0\|\le 2\bar\delta$ for all $i$, so $\|w_i(s)\|\le 2\bar\delta\|x_0(s)\|$ for all $s\in\mathbb{T}$, hence $\|w(s)\|_\infty \le 2\bar\delta\|x_0(s)\|$. Substituting into the bound of Theorem~\ref{th:main_theorem} gives \eqref{eq:iss_x0_bound}.
\end{proof}

This bound makes explicit how the leader trajectory and the heterogeneity level determine the ultimate synchronization accuracy.
